Allocating Opportunities in a Dynamic Model of Intergenerational Mobility

Opportunities such as higher education can promote intergenerational mobility, leading individuals to achieve levels of socioeconomic status above that of their parents. We develop a dynamic model for allocating such opportunities in a society that exhibits bottlenecks in mobility; the problem of optimal allocation reflects a trade-off between the benefits conferred by the opportunities in the current generation and the potential to elevate the socioeconomic status of recipients, shaping the composition of future generations in ways that can benefit further from the opportunities. We show how optimal allocations in our model arise as solutions to continuous optimization problems over multiple generations, and we find in general that these optimal solutions can favor recipients of low socioeconomic status over slightly higher-performing individuals of high socioeconomic status -- a form of socioeconomic affirmative action that the society in our model discovers in the pursuit of purely payoff-maximizing goals. We characterize how the structure of the model can lead to either temporary or persistent affirmative action, and we consider extensions of the model with more complex processes modulating the movement between different levels of socioeconomic status.

==> analysis.tex <==
%\section{Theoretical Analysis for $p_D \geq p_A$}
%\vspace{-2mm}
\section{Analysis}\label{sec:analysis}
%\vspace{-2mm}
In this section, we focus on settings in which $p_D \geq p_A$ and characterize the optimal policy to maximize the total discounted reward over generations. (We only provide the analysis for settings of $p_D = p_A$ but the extension to $p_D>P_A$ is straightforward). We cast the problem as deriving the infinite-time-horizon optimal policy in a continuous state- and action-space (Markov) Decision Process.
We characterize the optimal threshold and value function for every state $\phi_0 \in [0,1]$. Importantly, we show that there exists a tipping point $\phi^*_0$ that splits the state space into two distinct regions: states at which the optimal threshold uses strict affirmative action, and states at which the optimal policy consists of imposing equally high thresholds on both $A$ and $D$ groups. 


 \begin{figure*}[h!]
\centering
\begin{subfigure}[t]{0.3\textwidth}
  \centering
          \includegraphics[width=\textwidth]{Figures/Policy_Gamma_alpha_15_sigma_40_tau_10.png}
   \caption{The optimal $\theta_0$ at every state $0 \leq \phi_0 \leq 1$. \textbf{The optimal threshold decreases with $\phi_0$}. The dashed lines indicate the tipping points, $\phi^*_0$, below which $\sigma$ is the only optimal threshold, and above it $\sigma$ is not optimal.}\label{fig:policy_brief}
\end{subfigure}\hspace{2mm}
\begin{subfigure}[t]{0.3\textwidth}
  \centering
          \includegraphics[width=\textwidth]{Figures/AA_Gamma_alpha_15_sigma_40_tau_10.png}
        \caption{The difference between $\theta_0$ and $\theta_1$ at every state $0 \leq \phi_0 \leq 1$. The dashed lines specify the tipping points. Strict affirmative action is employed beyond $\phi^*_0$ only and \textbf{the extent of affirmative action is increasing in $\phi_0$}.}\label{fig:AA_brief}
\end{subfigure}\hspace{2mm}
\begin{subfigure}[t]{0.3\textwidth}
  \centering
          \includegraphics[width=\textwidth]{Figures/Convergence_Gamma_alpha_15_sigma_40_tau_10.png}
        \caption{The state to which the optimal policy converges given the initial state $\phi_0$. The dashed lines specify the tipping point, $\phi^*_0$. Note that \textbf{the optimal policy never shrinks the size of group $D$ to a value less than $\phi^*_0$}.}\label{fig:convergence_brief}
\end{subfigure}
\caption{Illustration of the (a) optimal policy, (b) extent of affirmative action, and (c) absorbing state.}
\end{figure*}
%
%\vspace{-3mm}
\xhdr{The Decision Process}\label{sec:DP}
Given $\alpha, \sigma, \tau$, and $\gamma$, we define a decision process $\cD_{\alpha, \sigma, \tau,\gamma} =(\Phi, \Theta, S, R)$ (or $\cD$ for short) with a continuous state space $\Phi=[0,1]$, action space $\Theta=[0,\sigma]$, state transition $S: \Phi \times \Theta \rightarrow \Phi$, and reward function $R: \Phi \times \Theta \rightarrow [0,1]$. Each state $\phi_0 \in \Phi$ corresponds to the fraction of disadvantaged individuals within the population. For instance, the states $0$ (or $1$) represents the population at the state where no one (or everyone) belongs to $D$. 
% 
The set of thresholds admissible in each state $\phi_0$ is denoted by $\Theta_{\phi_0}$.  $\Theta_{\phi_0}$ consist of all thresholds $0 \leq \theta_0 \leq \sigma$ that can satisfy the capacity constraint, $\alpha$. In other words, for any $\theta_0 \in \Theta_{\phi_0}$, if we impose the threshold $\theta_0 \in [0,\sigma]$ on group $D$, we can find a threshold $\theta_1 \in [0,\sigma+\tau]$ for group $A$ such that exactly $\alpha$ fraction of the overall population receives the opportunity. This capacity constraint translates into two conditions on $\Theta_{\phi_0}$. First, a threshold $\theta_0 \in \Theta_{\phi_0}$ should not give the opportunity to \emph{more than} $\alpha$ fraction of the population. Formally,
$\forall \theta_0 \in \Theta_{\phi_0}:  \phi_0 \left(1-\frac{\theta_0}{\sigma}\right) \leq \alpha$, which is equivalent to:
{%\footnotesize
\begin{equation}\label{eq:action_lb}
\forall \theta_0 \in \Theta_{\phi_0}: \quad \theta_0 \geq \sigma \left( 1 - \frac{\alpha}{\phi_0} \right).
\end{equation}
}
%
Second, a threshold $\theta_0 \in \Theta_{\phi_0}$ should not waste opportunities, that is, it should give the opportunity to \emph{at least} $\alpha$ fraction of the overall population. Formally,
$\forall \theta_0 \in \Theta_{\phi_0}:   \phi_0 \left(1-\frac{\theta_0}{\sigma}\right) + \phi_1 \geq \alpha.$
Replacing $\phi_1$ with $1-\phi_0$ and rearranging terms, the above is equivalent to
{%\footnotesize
\begin{equation}\label{eq:action:ub}
\forall \theta_0 \in \Theta_{\phi_0}: \quad  \theta_0 \leq \frac{\sigma(1-\alpha)}{\phi_0}.
\end{equation}
}
Figure~\ref{fig:actions} in the Appendix illustrates the actions satisfying conditions (\ref{eq:action_lb}) and (\ref{eq:action:ub}) for every state $\phi_0 \in [0,1]$.

\iffalse
\begin{figure}
  \begin{minipage}[c]{0.45\textwidth}
    \includegraphics[width=\textwidth]{Figures/actions.png}
  \end{minipage}\hfill
  \begin{minipage}[c]{0.45\textwidth}
    \caption{
       The admissible thresholds for every state of the decision process, $\cD$. The x-axis specifies the state $\phi_0$, and the y-axis highlights (in light red) the admissible thresholds, $\Theta_{\phi_0}$, at every state, $\phi_0$.
    } \label{fig:actions}
  \end{minipage}
\end{figure}
\fi

%\begin{figure*}[t!]
%	\centering
%		\includegraphics[width=0.5\textwidth]{Figures/actions.png}
%	\caption{The admissible thresholds for every state of the decision process, $\cD$. The x-axis specifies the state $\phi_0$, and the y-axis highlights (in light red) the admissible thresholds, $\Theta_{\phi_0}$, at every state, $\phi_0$.}
%	\label{fig:actions}
%\end{figure*}

The state transition function, $S: \Phi \times \Theta \rightarrow \Phi$, specifies the state transitioned to for every (state, admissible threshold) pair. Formally,
{%\footnotesize
\begin{equation}\label{eq:state}
\forall \phi_0 \in \Phi, \forall \theta_0 \in \Theta_{\phi_0}: \quad  S(\phi_0, \theta_0) = \phi_0 - \frac{\phi_0}{2\sigma} (\sigma^2 - \theta_0^2).
\end{equation}
}
The reward function, $R: \Phi \times \Theta \rightarrow [0,1]$, is defined as follows: $R(\phi_0, \theta_0)$ denotes the immediate reward of imposing threshold $\theta_0$ at state $\phi_0$ and is equal to: 
\iffalse
Formally,
$$\forall \phi_0 \in \Phi, \forall \theta_0 \in \Theta_{\phi_0}: \quad   R(\phi_0, \theta_0) = \frac{\phi_0}{2\sigma} (\sigma^2 - \theta_0^2)
+ \frac{\phi_1}{2\sigma} \left((\sigma+\tau)^2 - \theta_1^2\right).$$
Replacing $\phi_1$ with $1-\phi_0$ and $\theta_1$ with the right hand side of (\ref{eq:theta_1}), we obtain the following equivalent expression for $R$:
\fi
{%\footnotesize
\begin{equation}\label{eq:reward}
R(\phi_0, \theta_0) =  
\begin{cases}
\frac{\phi_0}{2\sigma} (\sigma^2 - \theta_0^2)
+ \frac{1-\phi_0}{2\sigma} \left((\sigma+\tau)^2 - \left( \frac{\sigma(1-\alpha) + (1-\phi_0)\tau - \phi_0 \theta_0}{1-\phi_0}\right)^2\right) \quad \forall \phi_0 \neq 1 \\
\frac{1}{2\sigma} (\sigma^2 - \theta_0^2) \quad \text{ for } \phi_0 = 1
\end{cases}
\end{equation}
}
%
%\vspace{-3mm}
\xhdr{Characterization of the Optimal Policy} 
Next, we illustrate and characterize the optimal policy for the decision process $\cD$ defined above. (For further information and references on continuous-state decision processes, see Appendix~\ref{app:continuous}.)
%
A deterministic policy $\pi$ for a decision process $\cD$ is a mapping $\pi: \Phi \rightarrow \Theta$
such that $\pi(\phi_0)$ prescribes the threshold at state $\phi_0$. The value $V_{\pi}(\phi_0)$ of a state $\phi_0$ under policy $\pi$ is the discounted reward of executing policy $\pi$ on $\cD$ starting with initial state $\phi_0$. A policy $\pi$ is optimal if its value function satisfies Bellman Optimality---defined recursively as:
{
\begin{equation}\label{eq:bellman}
V_{\pi}(\phi_0) = \max_{\theta_0} R(\phi_0, \theta_0) + \gamma V_{\pi}(S(\phi_0, \theta_0)).
\end{equation}
}
We establish in Appendix~\ref{app:value} that for our decision process $\cD$, the value function satisfying the above functional equation is \emph{unique}, \emph{continuous}, %\emph{decreasing}, \emph{concave},  
\emph{differentiable}, and \emph{decreasing}. (We prove these facts utilizing tools from recursive analysis and dynamic programming~\citep{stokey1989recursive,cotter2006non}). For simplicity, from this point on we refer to this unique optimal value function as $V(.)$ and drop the subscript $\pi$.

Let the correspondence $\Pi^*_0: \Phi \rightarrow 2^\Theta$ denote all optimal policies for $\cD$. More precisely, for any $0 \leq \phi_0 \leq 1$, the set $\Pi^*_0(\phi_0)$ contains all optimal threshold values at $\phi_0$.  
Figure~\ref{fig:policy_brief} illustrates $\Pi^*_0$ for a sample setting of the parameters $\alpha, \sigma, \tau, \delta$. (See Figure~\ref{fig:policy} in Appendix~\ref{app:analysis} for more instances.) Figure~\ref{fig:value} in the same Appendix illustrates the value function $V$. Note that the value function is consistently decreasing and concave.


%    \begin{figure}[b]
%        \includegraphics[width=0.3\textwidth]{Figures/Policy_Gamma_alpha_15_sigma_40_tau_10.png}
%   \caption{The optimal $\theta_0$ at every state $0 \leq \phi_0 \leq 1$. \textbf{The optimal threshold decreases with $\phi_0$}. The dashed lines indicate the tipping points, $\phi^*_0$, below which $\sigma$ is the only optimal threshold, and above it $\sigma$ is not optimal.}\label{fig:policy_brief}
%    \end{figure}\hspace{3mm}
%    \begin{figure}[b]
%        \includegraphics[width=0.3\textwidth]{Figures/AA_Gamma_alpha_15_sigma_40_tau_10.png}
%        \caption{The difference between $\theta_0$ and $\theta_1$ at every state $0 \leq \phi_0 \leq 1$. The dashed lines specify the tipping points. Strict affirmative action is employed beyond $\phi^*_0$ only and \textbf{the extent of affirmative action is increasing in $\phi_0$}.}\label{fig:AA_brief}
%    \end{figure}\hspace{3mm}
%    \begin{figure}[b]
%        \includegraphics[width=0.3\textwidth]{Figures/Convergence_Gamma_alpha_15_sigma_40_tau_10.png}
%        \caption{The state to which the optimal policy converges given the initial state $\phi_0$. The dashed lines specify the tipping point, $\phi^*_0$. Note that \textbf{the optimal policy never shrinks the size of group $D$ to a value less than $\phi^*_0$}.}\label{fig:convergence_brief}
%    \end{figure}
    

\iffalse
\begin{figure*}[t!]
    \centering
    \begin{subfigure}[b]{0.31\textwidth}
        \includegraphics[width=\textwidth]{Figures/Policy_Gamma_alpha_5_sigma_40_tau_5.png}
        %\label{fig:compas_dw}
    \end{subfigure}
    \begin{subfigure}[b]{0.31\textwidth}
        \includegraphics[width=\textwidth]{Figures/Policy_Gamma_alpha_15_sigma_40_tau_10.png}
        %\label{fig:compas_at}
    \end{subfigure}
    \begin{subfigure}[b]{0.31\textwidth}
        \includegraphics[width=\textwidth]{Figures/Policy_Gamma_alpha_15_sigma_40_tau_5.png}
        %\label{fig:compas_sw}
    \end{subfigure}
   \caption{The optimal policy $\theta_0$ at every state $0 \leq \phi_0 \leq 1$ for various settings of $\alpha, \sigma, \tau$, and $\gamma$. Note that in all cases, \textbf{the optimal threshold is monotonically decreasing with $\phi_0$}. Moreover, there exists a point below which $\sigma$ is the only optimal threshold, and above which $\sigma$ is no longer optimal. Observe that this point coincides with the tipping point, $\phi^*_0$, established in Theorem~\ref{thm:main} (depicted by dashed lines). The dotted red line illustrates the line of affirmative action, derived in Lemma~\ref{lem:AA-line}. Notice that \textbf{beyond $\phi^*_0$, the optimal policy is always below the line of affirmative action}.}\label{fig:policy}
\end{figure*}
%
\begin{figure*}[t!]
    \centering
    \begin{subfigure}[b]{0.31\textwidth}
        \includegraphics[width=\textwidth]{Figures/Scaled_Value_Gamma_alpha_5_sigma_40_tau_5.png}
        %\label{fig:compas_dw}
    \end{subfigure}
    \begin{subfigure}[b]{0.31\textwidth}
        \includegraphics[width=\textwidth]{Figures/Scaled_Value_Gamma_alpha_15_sigma_40_tau_10.png}
        %\label{fig:compas_at}
    \end{subfigure}
    \begin{subfigure}[b]{0.31\textwidth}
        \includegraphics[width=\textwidth]{Figures/Scaled_Value_Gamma_alpha_15_sigma_40_tau_5.png}
        %\label{fig:compas_sw}
    \end{subfigure}
   \caption{The scaled value function at every state $0 \leq \phi_0 \leq 1$ for various settings of $\alpha, \sigma, \tau$, and $\gamma$. The dashed lines specify the tipping point, $\phi^*_0$. Note that in all cases, \textbf{the value function is continuous, concave, and decreasing}.}\label{fig:value}
\end{figure*}
\fi

We say that the optimal policy, $\Pi^*_0$, uses affirmative action at a state $\phi_0$ if at $\phi_0$, it imposes a lower threshold on group $D$ compared to $A$. 
%
\begin{definition}[(Strict) Affirmative Action]
The optimal policy uses (strict) affirmative action at state $\phi_0$ if for all $\theta_0 \in \Pi^*_0(\phi_0)$ and all $\theta_1 \in \Pi^*_1(\phi_0)$, $\theta_0 < \theta_1$.
\end{definition}
If the inequality above is not strict (i.e., $\theta_0 \leq \theta_1$), we say the optimal policy uses \emph{weak} affirmative action.
%
Figure~\ref{fig:AA_brief} shows the extent of affirmative action for a sample setting of the parameters $\alpha, \sigma, \tau, \delta$. (See Figure~\ref{fig:AA} in Appendix~\ref{app:analysis} for more instances).

\iffalse
\begin{figure*}[t!]
    \centering
    \begin{subfigure}[b]{0.31\textwidth}
        \includegraphics[width=\textwidth]{Figures/AA_Gamma_alpha_5_sigma_40_tau_5.png}
        %\label{fig:compas_dw}
    \end{subfigure}
    \begin{subfigure}[b]{0.31\textwidth}
        \includegraphics[width=\textwidth]{Figures/AA_Gamma_alpha_15_sigma_40_tau_10.png}
        %\label{fig:compas_at}
    \end{subfigure}
    \begin{subfigure}[b]{0.31\textwidth}
        \includegraphics[width=\textwidth]{Figures/AA_Gamma_alpha_15_sigma_40_tau_5.png}
        %\label{fig:compas_sw}
    \end{subfigure}
   \caption{The difference between $\theta_0$ and $\theta_1$ at every state $0 \leq \phi_0 \leq 1$  for various settings of $\alpha, \sigma, \tau$, and $\gamma$. The dashed lines specify the tipping point, $\phi^*_0$. Note that strict affirmative action is only employed beyond $\phi^*_0$. Also note that \textbf{the extent of affirmative action is monotonically increasing in $\phi_0$}.}\label{fig:AA}
\end{figure*}
\fi

Our main result (Theorem~\ref{thm:main}) characterizes the states at which the optimal policy employs affirmative action. In particular, it establishes the existence of a tipping point $0 \leq \phi^*_0 \leq 1-\alpha$ that designate the region of affirmative action: At any state $\phi_0 \leq \phi^*_0$, the optimal policy assigns similar high threshold to both the advantaged and disadvantaged groups. In contrast, at any state $\phi_0 \leq \phi^*_0$ the optimal policy imposes a strictly lower threshold on group $D$ compared to $A$.
%
%\vspace{-2mm}
\begin{theorem}\label{thm:main}
Given $\alpha, \sigma, \tau, \gamma$ and the decision process $\cD$, let 
{%\footnotesize
\begin{equation}\label{eq:phi_star}
\phi^*_0 =  \max \left\{ 0, \min \left\{ 1-\alpha , 1 - \frac{\alpha \sigma}{2\tau} \left( 1 + \sqrt{1 + \frac{2\tau\gamma}{1-\gamma}} \right) \right\} \right\}.
\end{equation} 
}
\begin{itemize}
\item For any state $\phi_0 \leq \phi^*_0$, there exists $\theta_0 \in \Pi^*_0(\phi_0)$ and $\theta_1 \in \Pi^*_1(\phi_0)$ such that $\theta_0 = \theta_1$.
%\vspace{-2mm}
\item For any state $\phi_0 > \phi^*_0$, for all $\theta_0 \in \Pi^*_0(\phi_0)$ and all $\theta_1 \in \Pi^*_1(\phi_0)$ such that $\theta_0 < \theta_1$.
\end{itemize}
\end{theorem}
%\vspace{-2mm}
Next, we provide an overview of the proof for Theorem~\ref{thm:main}. 
The proof consists of establishing a series of Lemmas.
Lemma~\ref{lem:phi_0_star} determines the largest state $\phi^*_0 \in [0,1]$ below which the optimal policy consists of applying the high threshold of $\sigma$ to group $D$. Clearly, below such point, the optimal policy does not use affirmative action.  
%\vspace{-2mm}
\begin{lemma}[The Tipping Point]\label{lem:phi_0_star}
For any state $\phi_0 < \phi^*_0$, $\sigma \in \Pi^*_0(\phi_0)$.
\end{lemma}
%\vspace{-2mm}
We prove the above Lemma by utilizing \emph{backward induction}. (See Appendix~\ref{app:analysis} for the complete proofs.) Next, we investigate states larger than $\phi^*_0$. 
For every state $\phi_0 > \phi^*_0$, Lemma~\ref{lem:AA-line} identifies the set of thresholds that exhibit affirmative action. 
%\vspace{-2mm}
\begin{lemma}[Region of Affirmative Action]\label{lem:AA-line}
For a state $\phi_0^* < \phi_0 <1$, the threshold $\theta_0 \in \Pi^*_0(\phi_0)$ uses affirmative action if and only if $\theta_0 \leq \sigma(1-\alpha)+\tau(1-\phi_0)$.
\end{lemma}
%\vspace{-2mm}
Lemma~\ref{lem:AA-leq} establishes that the optimal policy uses weak affirmative action beyond $\phi^*_0$. That is, it shows that for any state $\phi_0 > \phi^*_0$, it is never optimal to impose a strictly higher threshold on D.% compared to A.
%\vspace{-2mm}
\begin{lemma}[Weak Affirmative Action]\label{lem:AA-leq}
Consider a state $\phi_0 >\phi^*_0$.
For all $\theta_0 \in \Pi^*_0(\phi_0)$ and all $\theta_1 \in \Pi^*_1(\phi_0)$, $\theta_0 \leq \theta_1$.
\end{lemma}
%\vspace{-2mm}
Proposition~\ref{prop:strict-AA} shows that beyond $\phi^*_0$, the optimal policy in fact uses \emph{strict} affirmative action. That is, at every state $\phi_0 > \phi^*_0$, the optimal policy imposes a strictly lower threshold on D compared to A. 
%\vspace{-2mm}
\begin{proposition}[Strict Affirmative Action]\label{prop:strict-AA}
Consider a state $\phi_0 >\phi^*_0$ with $V'(\phi_0) < 0$. for all $\theta_0 \in \Pi^*_0(\phi_0)$ and all $\theta_1 \in \Pi^*_1(\phi_0)$, $\theta_0 < \theta_1$.
\end{proposition}
%\vspace{-2mm}
%Proposition~\ref{prop:strict-AA} utilizes the fact that the derivative of the value function is always negative---which is established in Lemma~\ref{lem:value}.

\iffalse
Lemma~\ref{lem:phi_0_star} determines the state $\phi^*_0 \in [0,1]$ up to which $\sigma$ is an optimal threshold. Note that if $\sigma$ is an optimal threshold at a state $\phi_0$, the optimal policy does not use affirmative action at $\phi_0$. To see this, note that when $\sigma$ is optimal, any action $\theta_0 > \sigma$ is also optimal (they all pick a 0-fraction of group $D$ and are, therefore, effectively equivalent). %As the result, any $\theta_1 \geq \sigma$ is also an optimal threshold for the disadvantaged.   

\begin{lemma}[The Tipping Point]\label{lem:phi_0_star}
For any state $\phi_0 < \phi^*_0$, $\sigma \in \Pi^*_0(\phi_0)$.
\end{lemma}
\begin{proof}
We utilize \emph{backward induction} to pinpoint the largest state at which $\sigma$ is an optimal threshold.
First, observe that if $\phi_0$ if sufficiently small, $\sigma \in \Pi^*_0(\phi_0)$. To see this, note that at least for $\phi_0=0$, $\sigma \in \Pi^*_0(\phi_0)$. Second, note that if $\sigma \in \Pi^*_0(\phi_0)$), Bellman optimality (\ref{eq:bellman}) must hold:
\begin{eqnarray*}
V(\phi_0) &=&  R(\phi_0, \sigma) + \gamma V(S(\phi_0, \sigma)) \\
&=&  R(\phi_0, \sigma) + \gamma V(\phi_0),
\end{eqnarray*}
where in the second line we utilized the fact that $S(\phi_0, \sigma) = \phi_0$ for all $\phi_0 \in [0,1]$. This fact can be readily verified through (\ref{eq:state}).
Rearranging the above equation, we obtain:
$$V(\phi_0) = \frac{1}{1-\gamma}R(\phi_0, \sigma).$$
Replacing $R$ above with its definition (\ref{eq:reward}) and plugging $\sigma$ in place of $\theta_0$, we obtain:
\begin{eqnarray}\label{eq:value}
V(\phi_0) &=& \frac{1}{1-\gamma}\frac{1-\phi_0}{2\sigma} \left((\sigma+\tau)^2 - \left( \frac{\sigma(1-\alpha) + (1-\phi_0)\tau - \phi_0 \sigma}{1-\phi_0}\right)^2\right) \nonumber\\
&=& \frac{1}{1-\gamma}\frac{1-\phi_0}{2\sigma} \left((\sigma+\tau)^2 - \left( \frac{-\sigma\alpha + (1-\phi_0)\tau  + (1- \phi_0) \sigma}{1-\phi_0}\right)^2\right)\nonumber\\
&=& \frac{1}{1-\gamma}\frac{1-\phi_0}{2\sigma} \left((\sigma+\tau)^2 - \left(  \sigma + \tau - \frac{\sigma\alpha}{1-\phi_0}\right)^2\right)\nonumber\\
&=& \frac{1}{1-\gamma}\frac{1-\phi_0}{2\sigma} \frac{\sigma\alpha}{1-\phi_0} \left(2(\sigma+\tau) - \frac{\sigma\alpha}{1-\phi_0}\right)\nonumber\\
&=& \frac{\alpha}{(1-\gamma)} \left((\sigma+\tau) - \frac{\sigma\alpha}{2(1-\phi_0)}\right)
\end{eqnarray}
A corollary of the above is that
$$V(0) = \frac{\alpha}{(1-\gamma)} \left((\sigma+\tau) - \frac{\sigma\alpha}{2}\right).$$

Next, we derive the largest $\phi_0$ at which $\sigma$ remains an optimal threshold. Let's denote this point by $\tilde{\phi}_0$.
From Bellman optimality, we know that an action is optimal if and only if it is optimal with respect to the (optimal) value function. So taking (\ref{eq:value}) as the value function $V$ up to $\tilde{\phi}_0$, any optimal threshold at $\phi_0 \leq \tilde{\phi}_0$ must maximize $R(\phi_0, \theta_0) + \gamma V(S(\phi_0, \theta_0))$. Since $R(\phi_0, \theta_0) + \gamma V(S(\phi_0, \theta_0))$ is differentiable and $\tilde{\phi}_0$ is the largest state at which $\sigma$ is an optimal policy, $\sigma$ must satisfy the first order condition at $\tilde{\phi}_0$---that is, the partial derivative of $R(\phi_0, \theta_0) + \gamma V(S(\phi_0, \theta_0))$ (w.r.t. $\theta_0$) must be 0 at $(\tilde{\phi}_0, \sigma)$. 

We can derive the derivative of $R(\phi_0, \theta_0) + \gamma V(S(\phi_0, \theta_0))$ as follows:
\begin{equation}\label{eq:partial}
\dd{\theta_0} \left\{ R(\phi_0, \theta_0) + \gamma V(S(\phi_0, \theta_0)) \right\} =  \dd{\theta_0}  R(\phi_0, \theta_0) + \gamma \dd{\theta_0}\  S(\phi_0, \theta_0) \dd{\phi_0} V(S(\phi_0, \theta_0)).
\end{equation}
We can calculate each term in (\ref{eq:partial}) as follows:
\begin{eqnarray}\label{eq:partial_reward}
\dd{\theta_0} R(\phi_0, \theta_0) &=& -\frac{\phi_0\theta_0}{\sigma} + 
\frac{\phi_0}{\sigma} \left( \frac{\sigma(1-\alpha) + (1-\phi_0)\tau - \phi_0 \theta_0}{1-\phi_0}\right) \nonumber\\
&=&  \frac{\phi_0}{\sigma} \left( \frac{\sigma(1-\alpha) + (1-\phi_0)\tau - \phi_0 \theta_0}{1-\phi_0} - \theta_0\right) \nonumber\\
&=&  \frac{\phi_0}{\sigma} \left( \frac{\sigma(1-\alpha) + (1-\phi_0)\tau - \theta_0}{1-\phi_0} \right).
\end{eqnarray}
%
\begin{equation}\label{eq:partial_state}
\dd{\theta_0} S(\phi_0, \theta_0) = \frac{\phi_0\theta_0}{\sigma}.
\end{equation}
%
\begin{equation}\label{eq:partial_value}
\dd{\phi_0} V(\phi_0) = -\frac{\sigma \alpha^2}{2(1-\gamma)(1-\phi_0)^2}.
\end{equation}
Plugging (\ref{eq:state}), (\ref{eq:partial_value}), (\ref{eq:partial_reward}), and (\ref{eq:partial_state}) into (\ref{eq:partial}), we obtain that $\dd{\theta_0} \left\{ R(\phi_0, \theta_0) + \gamma V(S(\phi_0, \theta_0)) \right\}$ is equal to:
\begin{equation}\label{eq:derivative}
\frac{\phi_0}{\sigma} \left( \frac{\sigma(1-\alpha) + (1-\phi_0)\tau - \theta_0}{1-\phi_0} \right) 
- \gamma \frac{\phi_0\theta_0}{\sigma}
\frac{\sigma \alpha^2}{2(1-\gamma)(1-\phi_0 + \frac{\phi_0}{2\sigma} (\sigma^2 - \theta_0^2))^2}.
\end{equation}

As mentioned earlier, at $(\tilde{\phi}_0, \sigma)$, the derivative (\ref{eq:derivative}) must amount to 0. Therefore, to find $\tilde{\phi}_0$, we must solve the following equation (obtained by replacing $\theta_0$ in (\ref{eq:derivative}) with $\sigma$):
 \begin{eqnarray*}
&& 0 = \frac{\phi_0}{\sigma} \left( \frac{\sigma(1-\alpha) + (1-\phi_0)\tau - \sigma}{1-\phi_0} \right) 
- \gamma \phi_0
\frac{\sigma \alpha^2}{2(1-\gamma)(1-\phi_0)^2}\\
%
\left(\text{multiplying by } \sigma(1-\phi_0)^2/\phi_0) \right) &\Rightarrow & 0 =  (-\alpha\sigma + (1-\phi_0)\tau)(1-\phi_0) - \gamma\frac{\sigma^2 \alpha^2}{2(1-\gamma)}\\
%
&\Rightarrow & 0 = \tau (1-\phi_0)^2 - \alpha\sigma (1-\phi_0)
- \frac{\gamma\sigma^2 \alpha^2}{2(1-\gamma)} \\
%
%&\Rightarrow & 1-\phi_0 = \frac{\alpha \sigma}{2\tau} \left( 1 \pm \sqrt{1 + \frac{2\tau\gamma}{1-\gamma}} \right)\\
%
\end{eqnarray*}
Solving the above quadratic equation for $(1-\phi_0)$, we have:
\begin{equation*}
\tilde{\phi}_0 \in 1 - \frac{\alpha \sigma}{2\tau} \left( 1 \pm \sqrt{1 + \frac{2\tau\gamma}{1-\gamma}} \right)
\end{equation*}
To obtain the tightest bound, we pick the smaller value among the above two possibilities:
\begin{equation*}
\tilde{\phi}_0 = 1 - \frac{\alpha \sigma}{2\tau} \left( 1 + \sqrt{1 + \frac{2\tau\gamma}{1-\gamma}} \right)
\end{equation*}
Note that $\tilde{\phi}_0$ must always be between $0$ and $(1-\alpha)$ (due to the budget constraints illustrated in Figure~\ref{fig:actions}). So the above derivation only goes through if  $\tilde{\phi}_0 \leq (1-\alpha)$. Therefore, we have:
$
\phi^*_0 =  \max \left\{ 0, \min \left\{ 1-\alpha , \tilde{\phi}_0 \right\} \right\}.
$
\end{proof}
\fi



\iffalse
The following Lemma characterizes the region of affirmative action in the state-action space.
\begin{lemma}[Region of Affirmative Action]\label{lem:AA-line}
For a state $\phi_0^* < \phi_0 <1$, the threshold $\theta_0 \in \Pi^*_0(\phi_0)$ uses affirmative action if and only if $\theta_0 \leq \sigma(1-\alpha)+\tau(1-\phi_0)$.
\end{lemma}
\begin{proof}
Let $\theta$ be the threshold that if applied to both D and A at $\phi_0$, allocates opportunities exactly. We have that
$$\phi_0 \left(1-\frac{\theta}{\sigma} \right) + (1-\phi_0) \left(1-\frac{\theta-\tau}{\sigma} \right) = \alpha$$
or equivalently,
$$\theta = \sigma(1-\alpha)+\tau(1-\phi_0).$$
Note that $\theta_0 < \theta$ if and only if $\theta_1 > \theta$---otherwise the capacity constraints would not be maintained. Therefore, for any $\theta_0 < \theta$, $\theta_1>\theta_0$, which implies affirmative action.
%According to Lemma~\ref{lem:AA-leq}, we know that $\theta_0 \leq \theta_1$, so the only case when we won't have affirmative action is when $\theta_0 = \sigma(1-\alpha)+\tau(1-\phi_0)$.
\end{proof}
\fi



\iffalse
The following Lemma shows that beyond $\phi^*_0$, the optimal threshold for the disadvantaged is never higher than that for the advantaged.
\begin{lemma}[Weak Affirmative Action]\label{lem:AA-leq}
Consider a state $\phi_0 >\phi^*_0$.
For all $\theta_0 \in \Pi^*_0(\phi_0)$ and all $\theta_1 \in \Pi^*_1(\phi_0)$, $\theta_0 \leq \theta_1$.
\end{lemma}
\begin{proof}
Suppose not and there exists $\theta_0 \in \Pi^*_0(\phi_0)$ and $\theta_1 \in \Pi^*_1(\phi_0)$ such that $\theta_0 > \theta_1$. If we lower $\theta_0$ down to $\sigma(1-\alpha)+\tau(1-\phi_0)$ and increase $\theta_1$ up to $\sigma(1-\alpha)+\tau(1-\phi_0)$, we maintain the capacity constraints and at the same time achieve the following:
\begin{itemize}
\item[(a)] We improve the immediate reward of the current time step--- because we replace advantaged agents with low success probabilities in the range of $[\theta_1, \sigma(1-\alpha)+\tau(1-\phi_0)]$ with disadvantaged agents with higher success probabilities in $[\sigma(1-\alpha)+\tau(1-\phi_0), \theta_0]$.
\item[(b)] We move to a state with a relatively smaller size of group $D$ (simply because we gave the opportunity to more disadvantaged agents). The value function is strictly decreasing in $\phi_0$. Therefore, this new next state has a higher value compared to the previous one. 
\end{itemize}
The fact that we can improve the value contradicts the optimality of $\theta_0, \theta_1$. Therefore, $\theta_0 > \theta_1$ cannot hold
\end{proof}
\fi

\iffalse
The following Proposition establishes that beyond $\phi^*_0$, the optimal policy uses strict affirmative action.
\begin{proposition}[Strict Affirmative Action]\label{prop:strict-AA}
Consider a state $\phi_0 >\phi^*_0$. If $V'(\phi_0) < 0$, then for all $\theta_0 \in \Pi^*_0(\phi_0)$ and all $\theta_1 \in \Pi^*_1(\phi_0)$, $\theta_0 < \theta_1$.
\end{proposition}
\begin{proof}
Note that according to Lemma~\ref{lem:AA-leq}, for all $\theta_0 \in \Pi^*_0(\phi_0)$ and all $\theta_1 \in \Pi^*_1(\phi_0)$, $\theta_0 \leq \theta_1$. It only remains to show that the inequality is strict. That is, for all $\theta_0 \in \Pi^*_0(\phi_0)$ and all $\theta_1 \in \Pi^*_1(\phi_0)$, $\theta_0 \neq \theta_1$. 

Suppose not and there exists $\theta_0 \in \Pi^*_0(\phi_0)$ and $\theta_1 \in \Pi^*_1(\phi_0)$, such that $\theta_0 = \theta_1$. According to Lemma~\ref{lem:AA-line}, this implies that $\theta_0 = \sigma(1-\alpha)+\tau(1-\phi_0)$. Next we show that $\theta_0 = \sigma(1-\alpha)+\tau(1-\phi_0)$ cannot be an optimal threshold at $\phi_0$.

Recall that 
$$\Pi^*_0(\phi_0) = \arg\max_{\theta_0} R(\phi_0, \theta_0) + \gamma V(S(\phi_0, \theta_0)).$$
So if $\sigma(1-\alpha)+\tau(1-\phi_0) \in \Pi^*_0(\phi_0)$, it must satisfy the following first-order condition:
\begin{eqnarray*}
\dd{\theta_0} \left( R(\phi_0, \theta_0) + \gamma V(S(\phi_0, \theta_0)) \right) =  \dd{\theta_0}  R(\phi_0, \theta_0) + \gamma \dd{\theta_0}\  S(\phi_0, \theta_0) \dd{\phi_0} V(S(\phi_0, \theta_0)) = 0
\end{eqnarray*}
But note that $\dd{\theta_0} R(\phi_0, \theta_0)$ at $\theta_0 = \sigma(1-\alpha)+\tau(1-\phi_0)$ is 0:
\begin{eqnarray*}
\dd{\theta_0} R(\phi_0, \theta_0) &=&  \frac{\phi_0}{\sigma} \left( \frac{\sigma(1-\alpha) + (1-\phi_0)\tau - \theta_0}{1-\phi_0} \right) \\
&=&  \frac{\phi_0}{\sigma} \left( \frac{\sigma(1-\alpha) + (1-\phi_0)\tau - \left(\sigma(1-\alpha)+\tau(1-\phi_0)\right)}{1-\phi_0} \right) \\
&=&  \frac{\phi_0}{\sigma} \left( \frac{0}{1-\phi_0} \right) = 0
\end{eqnarray*}
So $\theta_0 = \sigma(1-\alpha)+\tau(1-\phi_0)$ can only be optimal if $\dd{\theta_0}\  S(\phi_0, \theta_0) \dd{\phi_0} V(S(\phi_0, \theta_0)) = 0$. But this equality cannot hold because
$\dd{\theta_0} S(\phi_0, \theta_0) = \frac{\phi_0\theta_0}{\sigma} > 0,$
%and according to Corollary~\ref{cor:value}, 
and $\dd{\phi_0} V(S(\phi_0, \theta_0)) < 0$. So $\theta_0 = \sigma(1-\alpha)+\tau(1-\phi_0)$ cannot be the optimal threshold at $\phi_0$.
\end{proof}
\fi

\iffalse
\begin{figure*}[b!]
    \centering
    \begin{subfigure}[b]{0.31\textwidth}
        \includegraphics[width=\textwidth]{Figures/Convergence_Gamma_alpha_5_sigma_40_tau_5.png}
        %\label{fig:compas_dw}
    \end{subfigure}
    \begin{subfigure}[b]{0.31\textwidth}
        \includegraphics[width=\textwidth]{Figures/Convergence_Gamma_alpha_15_sigma_40_tau_10.png}
        %\label{fig:compas_at}
    \end{subfigure}
    \begin{subfigure}[b]{0.31\textwidth}
        \includegraphics[width=\textwidth]{Figures/Convergence_Gamma_alpha_15_sigma_40_tau_5.png}
        %\label{fig:compas_sw}
    \end{subfigure}
   \caption{The state the optimal policy converges to with the initial state $\phi_0$. The dashed lines specify the tipping point, $\phi^*_0$. Note that \textbf{the optimal policy never shrinks the size of group $D$ to a value less than $\phi^*_0$}.}\label{fig:convergence}
\end{figure*}
\fi
%
%\vspace{-2mm}
\xhdr{Insights from the Analysis}
Next, we make several observations and remarks about the optimal policy.
First, note that the optimal policy never shrinks the size of $D$ to a value less than $\phi^*_0$. (See Figures \ref{fig:convergence_brief} and \ref{fig:convergence} for instances. For every initial state $\phi_0 \in [0,1]$, the plots show the state one converges to when the optimal policy is simulated for $1000$ steps on $\cD$.) In other words, affirmative action is optimal from a utilitarian point of view as long as group $D$ is sufficiently large. 

\iffalse
\begin{figure*}[t!]
    \centering
    \begin{subfigure}[b]{0.3\textwidth}
        \includegraphics[width=\textwidth]{Figures/gamma_star.png}
        \caption{ }
        \label{fig:gamma_star}
    \end{subfigure}
    \begin{subfigure}[b]{0.3\textwidth}
        \includegraphics[width=\textwidth]{Figures/tau_star.png}
        \caption{ }
        \label{fig:tau_star}
    \end{subfigure}
    \begin{subfigure}[b]{0.3\textwidth}
        \includegraphics[width=\textwidth]{Figures/alpha_star.png}
        \caption{ }
        \label{fig:alpha_star}
    \end{subfigure}
   \caption{
Visualizing the triples $(\alpha, \tau, \gamma)$ for which the
optimal policy uses persistent affirmative actions.
($\sigma = 1 - \tau$ for these plots.)
Points that lie above the surfaces in panels (a) and (c), and below
the surface in panel (b), correspond to parameter values yielding
persistent affirmative action.
(\ref{fig:gamma_star}) When $1-\frac{\alpha\sigma}{\tau}<0$, any $\gamma>0$ suffices for persistent affirmative action and eventually moving the entire population to group $A$. When $1-\frac{\alpha\sigma}{\tau}>0$, there exists some $\gamma < 1$ (and hence a finite level of patience) that suffices for persistent affirmative action. 
   (\ref{fig:tau_star}) When $\tau$ is sufficiently large, the optimal policy does not use persistent affirmative action; this is because for a large $\tau$, the extent of affirmative action required to pick up the best performing members of $D$ is large---which in turn significantly reduces the immediate reward. For any given value of $\alpha$, there exists a sufficiently small $\tau$ that guarantees persistent affirmative action.
   (\ref{fig:alpha_star}) When $\alpha$ is small relative to $\tau$, the optimal policy does not use persistent affirmative action, because the cost of picking the best performing members of $D$ is very high and a small $A$ group suffices for filling the available opportunities. Note that for some values of $\tau$, no matter how large $\alpha$ is, the optimal policy never uses persistent affirmative action.
   }\label{fig:star}
\end{figure*}
\fi
%
Second, the precise derivation of $\phi_0^*$ (\ref{eq:phi_star}) allows us to gain new insights into how the interaction between the parameters of our model can give rise to or avert affirmative action. 
Figure~\ref{fig:star} depicts the status of persistent affirmative action (i.e., $\phi_0^* \leq 0$) for $\alpha, \tau, \gamma$ in settings where $\sigma = 1-\tau$. (The derivation behind the plots can be found in Appendix~\ref{app:star}.) 
%Notice that persistent affirmative action is promoted by large values of $\alpha$ and small values of $\tau$. Moreover, a finite level of patience often suffices for persistent affirmative action.
%
%Figure \ref{fig:star} provides some ways of describing the regions of parameter space in which the optimal solution uses persistent affirmative action.
As the partitions of the space there make apparent, the interactions
among the key parameters is fairly subtle.
First, persistent affirmative action is promoted by large values of $\alpha$
and small values of $\tau$, since these make it easier to include 
high-performing members of group $D$ without a large difference in thresholds; 
and it is promoted by larger values of $\gamma$,
indicating greater concern for the rewards in future generations.
One might have suspected that persistent affirmative action would
only be realized as the optimal solution in the limit as society's
patience (essentially $\gamma / (1 - \gamma)$) goes to infinity;
but in fact, a sufficiently large finite amount of patience is sufficient for the optimal policy to use persistent affirmative action.
%
%\begin{proposition}[Absorbing State]
%For any $\phi_0>\phi^*_0$ as the initial state, the optimal policy converges to $\phi^*_0$. For any $\phi_0 \leq \phi^*_0$ as the initial state, the optimal policy stays at $\phi_0$.
%\end{proposition}
%\begin{proof}
%\hh{TBA.}
%\end{proof}

\iffalse
%\vspace{-3mm}
\xhdr{Optimal Policy for $p_A > p_D$}
The focus of our theoretical analysis here was on settings in which
$p_A \leq p_D$. When $p_A > p_D$, it becomes significantly more challenging to characterize the optimal allocation policy, in part because the backward induction technique no longer works. But we can
still approximately compute the optimal policy via discretization followed by
solution methods for finite MDPs. In Appendix~\ref{sec:sims}, we computationally investigate the optimal policy for setting in which $p_A > p_D$.  We observe two significant differences here: (a) the optimal policy can be \emph{non-monotone} in $\phi_0$. (b) There exists a \emph{sharp drop} in the optimal threshold at some intermediate state $\phi_0 \in [0,1]$. We interpret and discuss these empirical findings in Appendix~\ref{sec:sims}.
\fi

==> discussion.tex <==
\section{Discussion and Conclusion}\label{sec:discussion}

\paragraph{Summary} We developed and analyzed a model for allocating
opportunities in a society with limited intergenerational mobility.
These opportunities produce benefits in the present generation, but
they can also raise the socioeconomic status of the recipients
and their descendants.
This creates a trade-off: whether to maximize the current value achievable from the opportunities or to increase the value achievable
in future generations.
We have shown how to resolve this trade-off by solving a continuous
optimization problem over multiple generations, and we have seen
how optimal solutions to this problem can exhibit a form of
\emph{socioeconomic} affirmative action, 
favoring individuals
of low socioeconomic status over slightly higher-performing individuals
of high socioeconomic status.
Characterizing the conditions under which this type of 
affirmative action occurs provides insights into the
interaction between the amount of opportunity available,
the magnitude of the gap between different socioeconomic classes, 
and the ``patience''' of the society in evaluating the benefits
achievable from future generations. 






\paragraph{Impact and Ethical Considerations}
Our work addresses one potential role that (algorithmic) affirmative action policies can have on future generations and mitigating socioeconomic inequality. We follow a long tradition in the mathematical social sciences, where a stylized model is proposed to capture certain aspects of a complex societal issue; the model is then rigorously analyzed with the hope that the formal analysis provides new insights about alternative policy choices and their counterfactual effects. These insights can in turn inform policymakers at a qualitative level. 
All mathematical models are by definition highly simplified representations of the issues at hand, and as such it is important to understand and interpret them keeping their limitations and scope of applicability in mind. We have grounded our work in a broad literature from economics so as to draw on the insights that earlier modelers have brought to this setting. But we also apply the principle of acting with caution in drawing policy interpretations from mathematical models, and to this end, we shall next discuss the limitations of our work in detail. We hope that this discussion further illuminates the fact that theoretical models and their implications cannot and should not be taken as exact representations of the way complex societal processes operate and evolve. 

\paragraph{Limitations and Interpretations}
Our model is designed to model the tradeoff mentioned above in as simplified a fashion as possible; as such, it is important
to note some of its key limitations.
First, it is intended to model the effect of a single opportunity, and it treats other forms of mobility probabilistically in the background.
It also assumes that its fundamental parameters ($\alpha, \sigma, \tau, \gamma$) as constant over all generations.
It treats an individual's group membership ($A$ and $D$) and
ability as a complete description of their performance, rather than including any dependence on the group membership of the individual's parent. (That is, an individual in group $A$ performs the same in the model regardless of whether their parent belonged to group $A$ or $D$.)
All of these would be interesting restrictions to relax in an
extension of the model.

Much of the past theoretical work on intergenerational mobility focuses
on an issue that we do not consider here: the strategic considerations
faced by parents as they decide how much to consume in the present
generation and how much to pass on to their children.
Our interest instead has been in the optimization problem faced by
a social planner in allocating opportunities, treating the behavior of the agents as fixed and simple. Here too, it would be interesting to explore models that address these issues in combination. 
%
Moreover, because our focus is on intergenerational mobility in
a socioeconomic sense, we do not model discrimination based on race, ethnicity, or gender, and the role of race-based and gender-based affirmative action in combatting these effects.
The model is instead concerned with
\emph{socio-economic} or \emph{class-based}~\citep{malamud1995class,kahlenberg1996class} affirmative action.
That said, the ingredients here could be combined with models of statistical or taste-based discrimination on these attributes to better understand their interaction. 
%
The simplicity of our model, however, does allow us to make a correspondingly fundamental point: that even a purely payoff-maximizing society can discover affirmative action policies from first principles as
it seeks to optimize the allocation of opportunities over multiple 
generations.
Moreover, the optimal allocation policy is deeply connected
to dynamic programming over the generations;
the society is essentially attempting to ``steer'' the balance
of group $A$ and group $D$ over time, making sure not to turn things
too abruptly (giving up present benefit) or too gradually (giving up
future benefit).


\paragraph{Future Directions}
There are a number of interesting further research directions 
suggested by the results presented here and the limits of our model noted above. First, recall that according to our finding, the effectiveness of socioeconomic affirmative action depends of the
interaction between the amount of opportunity available,
the magnitude of the gap between different socioeconomic classes, 
and the society's patience. To understand where in this space any given society falls, a natural next step is to design algorithms for estimating or learning the value of these parameters given the appropriate data. 
Second, it would be interesting to consider extensions
of the model that allow basic parameters of the society to vary over
time; allow for multiple
opportunities being allocated concurrently; incorporate externalities among agents; and account of strategic consideration.
And finally, there is a natural opportunity to try integrating
the models here with work on the nature of statistical discrimination
and the design of interventions to alleviate it.

==> illustration.tex <==
%\subsection{Illustrations}
Figure~\ref{fig:policy} illustrates the optimal policy for several settings of the parameters. \hh{Further description TBD.}

\begin{figure*}[t!]
    \centering
    \begin{subfigure}[b]{0.32\textwidth}
        \includegraphics[width=\textwidth]{Figures/Policy_Gamma_alpha_5_sigma_40_tau_5.png}
        %\label{fig:compas_dw}
    \end{subfigure}
    \begin{subfigure}[b]{0.32\textwidth}
        \includegraphics[width=\textwidth]{Figures/Policy_Gamma_alpha_15_sigma_40_tau_10.png}
        %\label{fig:compas_at}
    \end{subfigure}
    \begin{subfigure}[b]{0.32\textwidth}
        \includegraphics[width=\textwidth]{Figures/Policy_Gamma_alpha_15_sigma_40_tau_5.png}
        %\label{fig:compas_sw}
    \end{subfigure}
   \caption{The optimal policy $\theta_0$ at every state $0 \leq \phi_0 \leq 1$ for various discount factors. The dashed lines specify the tipping point, $\phi^*_0$.}\label{fig:policy}
\end{figure*}

%\begin{figure*}[t!]
%    \centering
%    \begin{subfigure}[b]{0.32\textwidth}
%        \includegraphics[width=\textwidth]{Figures/Scaled_Value_Gamma_alpha_5_sigma_40_tau_5.png}
%        %\label{fig:compas_dw}
%    \end{subfigure}
%    \begin{subfigure}[b]{0.32\textwidth}
%        \includegraphics[width=\textwidth]{Figures/Scaled_Value_Gamma_alpha_15_sigma_40_tau_10.png}
%        %\label{fig:compas_at}
%    \end{subfigure}
%    \begin{subfigure}[b]{0.32\textwidth}
%        \includegraphics[width=\textwidth]{Figures/Scaled_Value_Gamma_alpha_15_sigma_40_tau_5.png}
%        %\label{fig:compas_sw}
%    \end{subfigure}
%   \caption{The scaled value function at every state $0 \leq \phi_0 \leq 1$ for various discount factors. The dashed lines specify the theoretical tipping point, $\phi^*_0$.}\label{fig:value}
%\end{figure*}

Figure~\ref{fig:AA} shows the extent of affirmative action for the same settings of parameters. \hh{Interpretation of the shape TBA.}
\begin{figure*}[t!]
    \centering
    \begin{subfigure}[b]{0.32\textwidth}
        \includegraphics[width=\textwidth]{Figures/AA_Gamma_alpha_5_sigma_40_tau_5.png}
        %\label{fig:compas_dw}
    \end{subfigure}
    \begin{subfigure}[b]{0.32\textwidth}
        \includegraphics[width=\textwidth]{Figures/AA_Gamma_alpha_15_sigma_40_tau_10.png}
        %\label{fig:compas_at}
    \end{subfigure}
    \begin{subfigure}[b]{0.32\textwidth}
        \includegraphics[width=\textwidth]{Figures/AA_Gamma_alpha_15_sigma_40_tau_5.png}
        %\label{fig:compas_sw}
    \end{subfigure}
   \caption{The difference between $\theta_0$ and $\theta_1$ at every state $0 \leq \phi_0 \leq 1$ for various discount factors. The dashed lines specify the theoretical tipping point, $\phi^*_0$.}\label{fig:AA}
\end{figure*}

Figure~\ref{fig:convergence} shows the state one converges to if the optimal policy is simulated (for $1000$ steps) on the MDP. \hh{more TBD.}
\begin{figure*}[t!]
    \centering
    \begin{subfigure}[b]{0.32\textwidth}
        \includegraphics[width=\textwidth]{Figures/Convergence_Gamma_alpha_5_sigma_40_tau_5.png}
        %\label{fig:compas_dw}
    \end{subfigure}
    \begin{subfigure}[b]{0.32\textwidth}
        \includegraphics[width=\textwidth]{Figures/Convergence_Gamma_alpha_15_sigma_40_tau_10.png}
        %\label{fig:compas_at}
    \end{subfigure}
    \begin{subfigure}[b]{0.32\textwidth}
        \includegraphics[width=\textwidth]{Figures/Convergence_Gamma_alpha_15_sigma_40_tau_5.png}
        %\label{fig:compas_sw}
    \end{subfigure}
   \caption{The state we converge to if we start with initial state $\phi_0$. The dashed lines specify the theoretical tipping point, $\phi^*_0$.}\label{fig:convergence}
\end{figure*}

==> introduction_old.tex <==
\section{Introduction}

Affirmative Action policies have been the subject of much debate. Proponents argue that such policies can restore fairness by incentivizing the historically-disadvantaged to invest in socially desirable qualifications (e.g., education). Opponents, on the other hand, argue that these policies divert society from the ideal of meritocracy. In addition to diminishing investment incentives, they bolster existing negative stereotypes against the historically-disadvantaged groups. With the rise of algorithmic decision-making systems in domains such as education and employment and their potential for unfairness and discrimination, these debates have come to the forefront of computer science research. 

In this work, we study the inter-generational impact of socio-economic affirmative action policies on the long-term welfare of society.
Consider a purely-utilitarian society solely interested in maximizing its long-term productivity/welfare---that is, the discounted utility over generations. Every individual in this society is born with an innate level of \emph{ability}---drawn uniformly at random---which determines their chance of productivity and success in the labor market if given the opportunity and resources (e.g., if admitted to college). In each generation, society consists of two socio-economic groups: the advantaged and the disadvantaged. Being a member of the advantaged group positively shifts one's likelihood of success. Society evolves from one generation to the next. The socio-economic status of an individual in the current generation stochastically determines that of their offspring in the next generation. 

How would such society allocate its opportunities and resources over time among advantaged and disadvantaged populations? Note that a myopic policy---which allocates all resources in each generation to individuals with the highest likelihoods of success---is not always optimal. While raising the allocation of opportunity to members of the disadvantaged group may reduce the productivity of the current generation, it expands the proportion of the advantaged population in future generations---which in turn boosts the productivity of those generations. This observation suggests that the optimal allocation of opportunities and resources in this society must strike a delicate balance between immediate- vs. future utility. 

As the canonical example, consider the case of \emph{college admissions}. One crucial factor in deciding whether to admit a student is his/her likelihood of graduating from college and succeeding in the labor market. This consideration may lead to favoring students who come from stabler socio-economic backgrounds. (Among students of similar ability and talent, those who come from stronger backgrounds are more likely to graduate from college). On the other hand, if we admit a student from a poor background, and they succeed, their achievement can have profound positive implications for their future generations. 


We characterize the conditions under which the optimal allocation policy employs affirmative-action---that is, it imposes a lower threshold on the disadvantaged compared to the advantaged. Importantly, we find that:
\begin{itemize}
\item A purely-utilitarian society can employ \emph{temporary} Affirmative Action policies to maximize its long-term welfare.
\item The relative size of the disadvantaged group impacts the extent of Affirmative Action.
Overall, the degree of affirmative action is monotonically increasing in the relative size of the disadvantaged population.
\item The society's level of patience influences the extent of Affirmative Action. A finite amount of patience suffices for Affirmative Action to \emph{persist} regardless of the relative size of the disadvantaged group.
\item If we weaken the effect of parental socio-economic status on determining their offspring's likelihood of success, we observe interesting non-monotonicities in the extent of Affirmative Action used by the optimal policy.
\end{itemize}

We must emphasize at the outset two essential issues that our work does \emph{not} attempt to address. 
First, while prior economic models of affirmative action focus on its \textbf{strategic} aspects, our model focuses on the optimal allocation of opportunities and resources over time. In particular, we do not address the role of \emph{stereotypes} in driving statistical discrimination and leading to socially undesirable equilibria.
Second, there is a vast literature on \textbf{race-based} and \textbf{gender-based} affirmative action policies, and \emph{race-sensitive admission policies} in the context of education. Our model is solely concerned with \emph{socio-economic} or \emph{class-based}~\citep{malamud1995class,kahlenberg1996class} affirmative action. In particular, our work does not weigh in on the intergenerational implications of racial identities and evolving social attitudes toward race. 

{\color{red}
\paragraph{Limitations}
\begin{itemize}
\item Focus on one opportunity alone, not considering other ways in which people's circumstance may change. One specific model of probabilistic movement. Other alternative imaginable.
\item Assuming that $\alpha$, $\sigma$, and $\tau$ are fixed through generations.
\item Don't model the impact of parental circumstance on their offspring (that is, once some one is in A, it doesn't matter whether their parent was in D or A).
\item Not modeling the real world, deliberately focusing on a stylized model of a selfish society that only cares about maximizing long-term discounted utility. 
\end{itemize}
}

\begin{figure*}[t!]
    \centering
    \begin{subfigure}[b]{0.32\textwidth}
        \includegraphics[width=\textwidth]{Figures/gamma_star.png}
        \caption{ }
        \label{fig:gamma_star}
    \end{subfigure}
    \begin{subfigure}[b]{0.32\textwidth}
        \includegraphics[width=\textwidth]{Figures/tau_star.png}
        \caption{ }
        \label{fig:tau_star}
    \end{subfigure}
    \begin{subfigure}[b]{0.32\textwidth}
        \includegraphics[width=\textwidth]{Figures/alpha_star.png}
        \caption{ }
        \label{fig:alpha_star}
    \end{subfigure}
   \caption{(\ref{fig:gamma_star}) When $1-\frac{\alpha\sigma}{\tau}<0$, any $\gamma>0$ suffices for persistant AA and eventually moving the entire population to the advantaged group. When $1-\frac{\alpha\sigma}{\tau}>0$, a finite level of patience $\left(\frac{\gamma}{1-\gamma}\right)$ suffices for persistant AA. 
   (\ref{fig:tau_star}) When $\tau$ is sufficiently large, the optimal policy does not use persistent AA, because for a large $\tau$, the extent of AA required to pick up any mass from D is large---which in turn significantly reduces the immediate payoff. Note that for any given value of $\alpha$, there exists a sufficiently small $\tau$ that guarantees persistent AA.
   (\ref{fig:alpha_star}) When $\alpha$ is small relative to $\tau$, the optimal policy does not use persistent AA, because again the cost of picking anyone from $D$ is very high and a small advantaged group suffices for filling the available opportunities. Note that for some values of $\tau$, no matter how large $\alpha$ is, we won't have persistent affirmative action.
   }\label{fig:star}
\end{figure*}

==> related-brief.tex <==
\subsection{Related Work}
We briefly mention several lines of scholarship that are closely related to our work. See Section~\ref{sec:related} for a more detailed discussion of related work.

\vspace{-2mm}
\xhdr{Intergenerational Income Mobility}
A substantial literature in economics addresses the relationship between income inequality and intergenerational mobility. At a high-level, the research suggests that higher inequality results in lower income mobility across generations (see, e.g.,~\citep{maoz1999intergenerational,corak2013income}). The precise measurements of inequality and mobility significantly influence the strength of this effect (see, e.g.,~\citep{solon1992intergenerational,piketty2000theories}). Existing work recognizes two main mechanisms through which a parent may affect its offspring income: (1) by transmitting endowments (e.g., innate abilities, connections, etc.) to the next generation; (2) by investing in the human capital of the next generation~\citep{becker1979equilibrium,solon1999intergenerational}. 
Theoretical models of income mobility study utility-maximizing parents who must decide how much of their capital to consume and how much of it to invest in their offspring~\citep{becker1986human,becker1979equilibrium,loury1981intergenerational,solon1999intergenerational}. As mentioned earlier, we deliberately set aside parental strategic considerations and focus on the optimal policy through the lens of a social planner interested in maximizing discounted payoff over generations.

\vspace{-2mm}
\xhdr{Affirmative Action Policies}
A rich body of work in economics investigates sources of statistical discrimination~\citep{arrow1973theory} and the role of affirmative action policies in redressing it. For an excellent survey of this literature, see~\citep{fang2011theories}. 
%
Outcome-based policies, such as affirmative action quotas, have long been proposed and implemented as \emph{temporary} remedies to eliminate group-level inequalities. Such policies are particularly effective when self-fulfilling stereotypes are the primary cause of group inequalities. Besides, a broader representation of minorities in higher social positions can generate role models who positively influence future generations in their investment decisions~\citep{chung2000role}. %Conversely, under certain conditions quota constraints may reduce the disadvantaged group's incentives to invest in skills, and subsequently, result in an worse asymmetric outcomes~\citep{coate1993will}.
%
While the economic literature on affirmative action mainly addresses \textit{race-based} interventions, some scholars have advocated for \emph{socioeconomic} or \emph{class-based} affirmative action as a race-neutral alternative (see, e.g., \citep{kahlenberg1996class,carnevale2013socioeconomic}). Race-neutral alternatives become particularly important to understand when race-sensitive interventions are constitutionally challenged (for example, see the case of Fisher v. University of Texas at Austin (2013)). 
The extent to which substituting socioeconomic status for race in
college admissions is effective in improving minority enrollment is contested (see, e.g., ~\citep{kane1998racial,reardon2006implications,gaertner2013considering,reardon2017can}). However, socioeconomic affirmative action can surely facilitate access to college for economically disadvantaged students. The resulting socioeconomic diversity is a desirable outcome in and of itself~\citep{reardon2017can} and in essence, it does not have to compete with or replace race-sensitive admission policies.
 


%\xhdr{Intergenerational Equity}
%
%\xhdr{Intergenerational Cultural Transmission}
%\citep{bisin2001economics} model the intergenerational transmission of preferences from parents to their offspring through socialization.  

\vspace{-2mm}
\xhdr{Long-term Implications of Fair Machine Learning} Several recent articles study the long-term impact of automated decision-making models and fairness interventions on society and individuals. \citep{hu2018short} and \citep{mouzannar2019fair} take inspiration from existing models of statistical discrimination and affirmative action. \citet{hu2018short} study the impact of enforcing statistical parity on hiring decisions made in a temporary labor market preceding a permanent one. \citet{mouzannar2019fair} model the dynamics of how a population reacts to a selection rule by changing their qualifications. \citet{liu2018delayed} and \citet{kannan2018downstream} study how a utility-maximizing decision-maker may respond to the predictions made by the model. %For instance, the decision-maker may interpret and use the predictions in a certain way, or update the model entirely. %\citet{heidari2019long} focus on how \emph{decision-subjects} respond to algorithmic predictions by improving/updating their qualifications. They propose a micro-scale behavioral model of how individuals update their qualifications by imitating their so-called role models------someone similar to them who has received a higher benefit.  %We don't make any case-specific assumptions about how the world changes in response to the deployed model, rather allow our micro-scale behavioral model to derive the macro-level change. %We emphasize that our model is not meant to perfectly capture all the behavioral nuances involved; rather our primary goal is to highlight the potential role of behavioral dynamics and human response in shaping the long-term impact of algorithmic models.  
%
% Strategic classification
\cite{dong2018strategic,hu2018disparate,milli2018social} address \emph{strategic classification}---a setting in which decision subjects are assumed to respond \emph{strategically} and potentially \emph{untruthfully} to the choice of the classification model, and the goal is to design classifiers that are robust to strategic manipulation. 
%
The above articles primarily focus on how the \emph{performance prediction} or \emph{evaluation} mechanism can incentivize the parties involved to respond strategically. In contrast, in our model, we make the simplifying assumption that performance prediction is perfectly accurate and instead concentrate on the optimal allocation of opportunities in society over time. 

